Towards Landau-Ginzburg models for cominuscule spaces via the exceptional cominuscule family

We present projective Landau-Ginzburg models for the exceptional cominuscule homogeneous spaces $\mathbb{OP}^2 = E_6^\mathrm{sc}/P_6$ and $E_7^\mathrm{sc}/P_7$, known respectively as the Cayley plane and the Freudenthal variety. These models are defined on the complement $X^\vee_\mathrm{can}$ of an anti-canonical divisor of the "Langlands dual homogeneous spaces" $\mathbb{X}^\vee = P^\vee\backslash G^\vee$ in terms of generalized Pl\"ucker coordinates, analogous to the canonical models defined for Grassmannians, quadrics and Lagrangian Grassmannians in arXiv:1307.1085, arXiv:1404.4844, arXiv:1304.4958. We prove that these models for the exceptional family are isomorphic to the Lie-theoretic mirror models defined in arXiv:math/0511124 using a restriction to an algebraic torus, also known as the Lusztig torus, as proven in arXiv:1912.09122. We also give a cluster structure on $\mathbb{C}[\mathbb{X}^\vee]$, prove that the Pl\"ucker coordinates form a Khovanskii basis for a valuation defined using the Lusztig torus, and compute the Newton-Okounkov body associated to this valuation. Although we present our methods for the exceptional types, they generalize immediately to the members of other cominuscule families.

==> toclayout.tex <==
\makeatletter
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\@M
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax \advance\leftskip\@tempdima\relax
    \rightskip\@pnumwidth plus4em \parfillskip-\@pnumwidth
    #5\leavevmode\hskip-\@tempdima
      \ifcase #1
       \or\or \hskip 1em \or \hskip 2em \else \hskip 3em \fi%
      #6\nobreak\relax
    \hfill\hbox to\@pnumwidth{\@tocpagenum{#7}}\par% <---- \dotfill -> \hfill
    \nobreak
    \endgroup
  \fi}
\makeatother
